Single Machine Graph Analytics on Massive Datasets Using Intel Optane DC Persistent Memory

Intel Optane DC Persistent Memory (Optane PMM) is a new kind of byte-addressable memory with higher density and lower cost than DRAM. This enables the design of affordable systems that support up to 6TB of randomly accessible memory. In this paper, we present key runtime and algorithmic principles to consider when performing graph analytics on extreme-scale graphs on large-memory platforms of this sort. To demonstrate the importance of these principles, we evaluate four existing shared-memory graph frameworks on large real-world web-crawls, using a machine with 6TB of Optane PMM. Our results show that frameworks based on the runtime and algorithmic principles advocated in this paper (i) perform significantly better than the others, and (ii) are competitive with graph analytics frameworks running on large production clusters.

==> background.tex <==
%We focus on two concerns in this paper. The first
%is graph analytics on large graphs that may not fit in the main memory
%of a machine (Section~\ref{large-graphs}).  The second is algorithm
%design for efficient data accesses in graph analytics to avoid
%negative caching effects during computation (Section~\ref{efficient-access}).
%
%Once the graph
%is in memory, in order to get good performance, the graph analytics system
%should optimize accesses to memory based on the underlying architecture to
%avoid degrading performance due to bad cache behavior.

Graph analytics does processing on graphs in order derive useful
properties about the graph for the user.
In Section~\ref{compute-graph}, we detail how graph analytics is done.
In Section~\ref{large-graphs}, we detail how to process large graphs
when the memory on a single machine is not sufficient.

\subsection{Computation on Graphs}
\label{compute-graph}
Graphs are represented as a set of nodes and their edges. Each node
as labels representing current execution state, and program
execution consists of updating said labels in some structured
manner using both the current labels of the nodes as well as the
edges in the graph.  Updates can be represented by a computation
rule called an \emph{operator}~\cite{pingali11} that is applied onto
a node. The operator takes the labels of a node and updates itself
and/or the labels of the neighborhood of that node, where
the neighborhood is defined in the operator and is not necessarily
immediate neighbors of the node. Vertex programs are set of graph
analytics applications where the operator neighborhood consists
only of immediate neighbors of a node: more general graph applications
may use less restricted neighborhoods, and this can allow for more
efficient algorithms. Operators are applied to nodes in the graph until
some termination condition is met, at which point the algorithm ends.

In order to operate on the graph, the structure of the graph that is being
operated on should be in memory. Graph analytics systems such as
Ligra~\cite{ligra}, Galois~\cite{galois}, or GraphIt~\cite{graphit} will
load the entire graph into memory before computation occurs so that any kind
of computation will not need to load anything more from disk.

\subsection{Handling Large Graphs}
\label{large-graphs}

Graph analytics systems that load an entire graph into memory to operate on it
will be referred to as \emph{shared-memory} systems in this paper. The problem
with them is that they are limited by the amount of memory present on the
machine: if you cannot load a large graph due to memory constraints,
you cannot operate on it.

There are two main approaches to processing large graphs: (1) avoid loading
the entire graph into memory and load only what is necessary
or (2) distribute the graph among many machines
(therefore increasing the total amount of memory a system has to work with)
and run the graph computation in a distributed manner.

\subsubsection{Out-of-core}
In \emph{Out-of-core} graph analytics systems, the graph resides on the secondary storage (SSD/disk)
and portions of the graph are read into DRAM under software control for in-memory processing.
%do not load the entire graph into memory, but instead, they load small portions of the graph into memory and
%operate on that portion of the graph before moving on to the next.
The state-of-the-art systems in this space include Graph- Chi~\cite{graphchi}, X-Stream~\cite{xstream},
GridGraph~\cite{gridgraph}, and BigSparse~\cite{bigsparse}.
Secondary storage devices have large access latencies and are block-addressable which favor sequential accesses.
Therefore, the main focus of \emph{Out-of-core} frameworks is to avoid repeated or random accesses
during computation for good performance.
\emph{Out-of-core} systems are generally orders of magnitude slower than shared-memory systems
if the graph
%shared-memory system
can fit in memory. Additionally, preprocessing of
the graph may need to be done in order to organize the data in a layout
that is friendly for the out-of-core system to run on.

% For efficiency, \emph{Out-of-core} tries to these systems need to have a structured
% manner of loading and storing data in order to
% %so that they
% avoid repeated or random disk accesses which can add large overhead to a graph computation.
% For example, they may store node data in the order that they are accessed on disk and may
% sort the edges of the nodes such that accesses to the data of the edge
% destinations are also sequential on disk~\cite{graphchi}. Some systems may even
% store node data in memory and only load in edge data as it is
% required~\cite{gts}.

%The downside of these systems is that they add disk overhead to the computation
%of an algorithm and

\subsubsection{Distributed-Memory}
\emph{Distributed-memory} graph analytics systems use distributed-memory clusters that
have sufficient main memory for in-memory processing of the graphs.
The graph is partitioned
%the graph
among many machines in a cluster using various partitioning policies~\cite{partitioningstudy}.
%and do the graph computation in a distributed manner.
Since the graph is now located on many different machines, there is communication
involved during graph computation in order to synchronize the updates
of a graph algorithm across all machines. Generally, these systems create
cached-copies of nodes and sychronize the cached copies periodically throughout
execution.
%~\cite{gluon}.
The state-of-the-art systems in this space include
PowerLyra~\cite{powerlyra}, D-Galois~\cite{gluon}, and Gemini~\cite{gemini}.
\emph{Distributed-memory} graph analytics systems not only allow users to process large
graphs, but also execute very fast due to in-memory processing and extra computation
power that comes with multiple machine in a cluster.
The main focus of \emph{Distributed-memory} graph analytics systems is to optimize the communication
as it often becomes the main bottleneck is distributed graph analytics~\cite{gluon, gemini}.

% In addition to the additional memory gained by running on multiple machines,
% these systems also benefit from the increased computational power of running
% an algorithm in parallel on multiple machines. Therefore, computation time on
% these systems is generally less than that on shared-memory or out-of-core
% systems. However, total execution time may not be less than other systems
% because there is now communication time to consider: communication overhead is
% the main overhead in distributed graph applications~\cite{gluon}.

% To improve performance in distributed-memory systems, care must be taken
% to optimize the communication~\cite{gluon} or partition the graph in such a
% way that communication is minimized~\cite{partitioningstudy}. Even then,
% it is difficult to find a single best partitioning policy for all
% algorithms~\cite{partitioningstudy}, and running on a distributed cluster is
% not nearly as accessible as running on a single machine.

Both \emph{Out-of-core} and \emph{Distributed-memory} graph analytics systems, however,
generally cannot directly run programs written for shared-memory graph analytics expecting
the same performance: it is usually necessary to rethink algorithms and data structures
from scratch.


==> results_3dxpointBenefits.tex <==

\subsection{Medium-size graphs: using \xpointshort vs. DDR4 DRAM}
\label{subsec:xpoint_vs_dram}

Recall that the DDR4 DRAM available on the machine we use is 384GB.
Two of our graphs (Table~\ref{tbl:inputs}), kron30 and clueweb12,
fit in the DRAM available (using Galois), so we evaluate these graphs using DRAM.
We choose the algorithms in Galois that perform best on 96 threads
(including new ones we implemented, so the execution time may be faster
than in Figure~\ref{fig:res:other_vs_galois}).
Figure~\ref{fig:res:dram_vs_xpoint} shows the strong scaling of all benchmarks
in Galois for these graphs on DRAM only and \xpointshort (with DRAM as cache).
kron30 requires $\sim136$GB which is $3\times$ smaller than the DRAM
available, so \xpointshort delivers performance almost identical to DRAM
by caching it in DRAM effectively. On the other hand, clueweb12 requires $\sim365$GB which is quite close to the DRAM available, thereby leading to significantly
more conflict-misses (\todo{$?\%$}) in the near-memory of \xpointshortend.
Another trend is that for threads $\leq 24$, \xpointshort can be much slower than DRAM
due to the way Galois allocates memory. Both interleaved and blocked allocation policies in Galois interleave and block, respectively, among the threads and not among the sockets.
Consequently, for threads that fit in a single socket ($\leq 24$),
the entire memory ends up being allocated on a single socket,
thereby leading to conflict-misses in near-memory.
This can be overcome by using different allocation policies
based on the number of threads. On 96 threads, \xpointshort can take up to 65\% more execution time than DRAM. On average, it takes only $7.3\%$ more time than DRAM.

% Figure~\ref{fig:res:dram_vs_xpoint} compares the \xpointshort performance with DRAM for kron30 and
% clueweb12 as well as shows the scaling with the number of threads. For each application, we measured the execution time when (a) the graph is stored entirely
% in DRAM only (not using \xpointshort by configuring 0\% of \xpointshort in Memory mode) and when (b) the graph is stored entirely in \xpointshort(100\% of \xpointshort is configured in the
% memory mode) at the start of the computation and cached into near-memory (DRAM in this case) as needed .

% Results show that for graphs which easily fit in the DRAM available on the machine like kron30
% (kron30 (136GB) is 3$\times$ smaller than the DRAM available on the machine (384GB)), \xpointshort can deliver performance identical to DRAM. For clueweb12 (365GB), which is the
% largest graph that we could fit on our machine, there is performance degradation on \xpointshort as comapred to DRAM. We observe apporx.
% 25\% (geomean) slowdown across all the benchmarks at 96 threads. The main reason for this slowdown is the
% increase in the conflict misses in the near-memory (DRAM) as the memory footprint approaches the size of available near-memory.
% Another trend to note is that the slowdown is
% higher for threads less than 24, which is due to the way Galois allocates memory using application-level NUMA aware policy. Since threads less than or equal to 24 are all on a
% single socket, Galois allocates the entire memory on a that particular socket using \texttt{first-touch} policy by making active threads touch the pages, which harms the performance on \xpointshort as explained in~\ref{subsub:numa_policy}.

\subsection{Very large graphs: using \xpointshort vs. a Cluster}
\label{subsec:xpoint_vs_stampeded}
% The size of the input graphs handled by the shared memory graph analytics is limited by the amount of
% memory present on the system. \xpointshort presents an exciting alternative to do graph analytics on massive graphs as shared memory graph analytics framework can be used
% out-of-the-box. The other methods commonly employed for large graphs are (a) distributed-memory graph analytics~\cite{powergraph, powerlyra, gemini,gluon} using
% distributed cluster or (b) out-of-core graph analytics~\cite{graphchi, xstream, gridgraph} using secondary storage devices as described in section~\ref{sec:background}.
%
%  To process graphs with billions of nodes and edges, one of the following
% methods are commonly employed: (a) Use distributed-memory clusters that have sufficient main memory for
% in-memory processing of the graphs. Another reason to go distributed is to get more compute resources. The state-of-the-art systems in this space include PowerGraph~\cite{powergraph}, PowerLyra~\cite{powerlyra}, Gemini~\cite{gemini}, and D-Galois~\cite{gluon}. (b) Another way to handle large graphs is to use
% out-of-core processing in which graphs reside on secondary storage and portions of the graph are read
% into DRAM under software control for in-memory processing. GraphChi~\cite{graphchi}, Xstream~\cite{xstream},
% and GridGraph~\cite{gridgraph} are state-of-the-art in this space. For both of the above mentioned solutions, in-memory graph-analytics programs cannot be used directly, and it is usually necessary to rethink algorithms and data structures from scratch.
%
% Distributed-memory graph analytics frameworks are usually orders of magnitude faster than out-of-core graph analytics
% as out-of-core solutions are limited by the secondary storage (disk/SSD) bandwidth. Therefore, we will
% compare shared memory graph analytics on \xpointshort using Galois with state-of-the-art distributed graph analytics
% framework, D-Galois~\cite{gluon}.
%
To evaluate distributed execution, we use the state-of-the-art
distributed graph analytics framework, D-Galois~\cite{gluon}.
D-Galois uses the same computation runtime as Galois, but
its programming model is more restricted to support efficient communication,
so the benchmarks provided by D-Galois do not use the same algorithms
as those in Galois.
D-Galois also uses implicit dense worklists unlike Galois, and
we use the D-Galois benchmarks without modifications.
We implemented these algorithms in Galois for \xpointshort
using sparse worklists, and we use the best-performing algorithm in Galois.
We evaluate D-Galois on a production cluster, Stampede2.
Based on recommendations from a prior study~\cite{partitioningstudy},
we use Outgoing Edge Cut (OEC) policy for 5 and 20 hosts
and Cartesian Vertex Cut (CVC) policy for 256 hosts to partition the
graphs. We exclude graph loading, partitioning, and construction time.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Stampede2 provides access to much more compute resources than the
%\xpointshort machine we use,
%so we also experiment with different compute resources.

Figure~\ref{fig:res:stampede_vs_xpoint_same_cores} compares
the performance of Galois on \xpointshort machine with that of
D-Galois on the Stampede2 distributed cluster
for all benchmarks on clueweb12, uk14, and wdc12.
First, we compare the performance using the same algorithm and
same amount of compute resources (80 threads) on both \xpointshort and Stampede2.
For distributed execution, we used the minimum number of hosts required to
fit the graph in-memory (5 hosts for clueweb12 and uk14, and 20 hosts for
wdc12) and restricted the number of threads on each host
(16 threads each on clueweb12 and uk14, and 4 threads each for wdc12).
% to get a total of 80 threads for a fair comparison.
These results are bars \textbf{DS} (Distributed Same) and
\textbf{OS} (Optane Same) in Figure~\ref{fig:res:stampede_vs_xpoint_same_cores}.
We observe that in most cases, \textbf{OS} is either similar or better than \textbf{DS}.
The most notable exception to this is pr.
D-Galois partitions the graph among the hosts,
which may lead to better spatial locality on each host.
Spatial locality reduces the computation time significantly for
topology-driven algorithms like pr, so D-Galois is faster than Galois for pr.
The performance of Galois for pr can be improved by using similar partitioning
for caches (like segmented subgraphs in GraphIt~\cite{graphit}).
% since distributed execution used residual based pagerank pull version which gives better performance in distributed setting as it minimizes the communication. It incurs lots of memory access, which is detrimental to shared memory execution.
Nevertheless, \textbf{OS} is 1.9$\times$ faster than \textbf{DS} on average
for all inputs and benchmarks.

We next compare same algorithm on the two platforms
but do not restrict the number of cores for Stampede2 and \xpointshortend.
These are the bars \textbf{DM} (Distributed Minimum) and
\textbf{OA} (Optane All), respectively.
Excluding pr, \textbf{OA} is 1.3$\times$ faster on average than \textbf{DM}
even though Stampede2 is using more compute resources than \xpointshort
(2.5$\times$ faster for clueweb12 and uk14, and 10$\times$ faster for wdc12).

The bar \textbf{OB} (Optane Best) represents the best-performing algorithm
for Galois; the algorithms reduce the number of memory accesses by
being more work-efficient.
These algorithms either cannot be implemented in D-Galois
(they are difficult to implement in distributed-memory, even by experts),
or they do not perform better than the algorithm used by D-Galois on
distributed execution.
\textbf{OB} is 2.6$\times$ faster on average than \textbf{DM}, excluding pr.

Finally, the bar \textbf{DB} (Distributed Best)
shows the performance on 256 Stampede hosts (12288 cores),
and we observe that \textbf{OB} either matches or performs better than
\textbf{DB} for bc, bfs, kcore, and sssp. For these benchmarks,
distributed execution does not scale that well,
so additional compute resources do not yield much benefit.

The main takeaway from these results is that \xpointshort
enables us to perform analytics on massive graphs using existing
frameworks out-of-the-box while yielding performance comparable or
better than that of a distributed cluster.
Thus, it boosts both programming productivity as well as performance.


==> results_3dxpointSetup.tex <==
A key benefit of \xpointshort in that in Memory Mode, it enables running 
shared-memory applications without significant modifications to work on massive datasets.
However, the systems issues identified in Section~\ref{3dxpoint} must be addressed
as described below.

\subsubsection{NUMA Allocation Policy}

%In modern multi-socket system, NUMA-aware data placement can significantly
%enhance the application performance by increasing the overall bandwidth and
%reducing the latency to memory. Due to the widespread presence of NUMA systems,
%the majority of operating system kernels, such as Linux~\cite{linux}, provides
%NUMA support that understands the topological properties of the system's memory
%in order to provide reproducible and better performance.
%Similar to the DRAM distribution in NUMA systems,
%the \xpointshort modules are also distributed
%among sockets.  Figure~\ref{fig:3dxpoint_diagram} shows an example of 2 socket
%machine with 384GB of DRAM and 6TB of \xpointshortend.
%Another important thing
%to note about \xpointshort NUMA systems is that \xpointshort modules
%on a given socket can only use the DRAM present in its local NUMA node as
%its last-level of cache (also know as near-memory).
%A good NUMA allocation policy on DRAM systems simply tries to allocate memory
%local to the cores on a NUMA node as it increases the overall bandwidth
%and reduces the memory access latency. This can be achieved by using Linux
%utilities such as \texttt{numactl} or by handling NUMA allocation inside
%the application using policies like \texttt{first-touch} where pages are
%allocated on the socket local to the cores first accessing them.
%\xpointshort, on the other hand,
%has to take another factor into account: the near-memory hit rate.
%The cost of near-memory miss is much higher than the remote NUMA access,
%and thus, it plays important role on data placement in \xpointshort system.
%It is more beneficial to allocate memory such that system can utilize more
%DRAM as near-memory even if it means more remote NUMA accesses.




\subsubsection{NUMA Migration}

%\subsubsection{NUMA Migrations are more harmful on Optane DC PMM:}
%If the OS level NUMA allocation policy is not specified, the OS (Linux) can
%dynamically migrate data between NUMA nodes in order to maximize the local
%NUMA accesses. This can also happen when application level NUMA policy which
%is not visible to the OS, such as \texttt{first-touch}, is used.
%NUMA page migrations are helpful in case of multiple applications sharing a
%single system as it tries to move pages closer to the cores assigned
%to the application. However, for single application running on the machine,
%it may not always be useful, especially when application has
%specified its own NUMA allocation policy depending on the knowledge of its
%memory access pattern.
%
%OS-directed migrations has overheads: (a) it requires book-keeping to keep
%track of the accesses to the pages to select pages for migration,
%(b) migration changes the virtual-to-physical address mapping, which makes
%the Page Table Entires (PTEs) cached in CPU's translation
%Lookaside Buffers(TLBs)\footnote{TLBs are hardware structures that cache
%recently used page table entries to assist virtual-to-physical
%address translation by avoiding page walks. Typically, each CPU core
%has its own TLB hierarchy.} stale and, therefore, requires TLB
%shootdown on each core. TLB shootdown involves slow operations such as issuing
%inter-process-interrupts (IPIs), and it increases TLB misses. Researchers have
%also looked at the impact of page granularity on migration overhead as
%well~\cite{arka18}. NUMA migrations in Linux can easily be turned off by
%setting a flag \texttt{numa\_balancing} in the kernel.


\subsubsection{Page Size}

%As computer system main memory sizes and workload sizes grow, the time spent
%handling TLB misses could become a performance bottleneck as large working
%sets necessitate many address translations. This bottleneck can be tackled by
%(a) increasing the TLB size in the hardware or by (b) increasing the page size.
%Increasing the TLB size is expensive and increases processor die area. On
%the other hand, increasing page size is cheaper. Also, fixing a page size is
%not desirable as different page sizes work best for different types of
%workloads. Therefore, processors today support various page sizes as well as
%separate TLBs for each size; for example, x86 supports traditional
%4KB small pages as well as 2MB and 1GB huge pages.

We studied the impact of page size for graph analytics applications
% on massive graphs for both \xpointshort and DDR4 DRAM
for a 4KB small page size and a 2MB huge
page size. Figure~\ref{fig:res:numa_migration_benchmark} shows the performance of bfs
(similar behavior was observed for other benchmarks) using Galois
for various large graphs
on (a) \xpointshort and (b) DDR4 DRAM.
NUMA migration is turned off and Galois uses NUMA interleaved for bfs.
% both without NUMA page migrations for fair
% comparison as the page migration overheads are higher for small page size as
% explained in the previous section~\ref{subsubsec:numa_migrations}.
% The system on which this was evaluated consisted of Data TLB with 4-way,
% 64 entries for 2KB pages and 4-way, 32 entries for 2MB pages. The 2MB huge
% pages were used by reserving memory for huge pages\footnote{In
% Linux, memory can be reserved for huge pages by writing the number of desired
% pages to \texttt{/proc/sys/vm/nr\_hugepages} using root privileges.} and
% passing \texttt{MAP\_HUGETLB} flag to \texttt{mmap}.
We observe that using huge
pages is always beneficial for graph analytics applications on large input
graphs
% on both \xpointshort as well DRAM
as huge pages reduce the number of the
number of pages required by 512$\times$, which reduces the number of TLB misses
(3.2$\times$ for clueweb12 and 1.9$\times$ for wdc12 as seen in
Table~\ref{tbl:page_size_counters}) and CPU cycles spent on page
walking on TLB misses (7.3$\times$ for clueweb12 and 8.8$\times$ for wdc12 as
seen in Table~\ref{tbl:page_size_counters}). We also observe that benefits of
huge pages are higher on \xpointshort as compared to DRAM as
% near-memory is used as direct-mapped cache~\footref{fn:tlb}. Therefore,
TLB misses also increase the near-memory access latency.
% The main takeaways from the above observations are
% (a)
Huge pages increase the TLB
reach\footnote{TLB reach = (TLB size $\times$ Page size).},
thereby reducing the TLB misses.
Thus, they are critical for reducing the cost of accesses in \xpointshortend.
% (b) huge pages are particularly
% beneficial for systems with large direct mapped cache such as near-memory in
% \xpointshort as TLB misses add to the near-memory (cache) access latency.


==> results_algorithms.tex <==
\begin{figure}
    \centering
    %\begin{minipage}{\textwidth}
    \begin{minipage}{0.49\textwidth}
        \centering
    \includegraphics[width=\textwidth]{algo_comparison_bfs}
    (a) bfs
    \end{minipage}
    \begin{minipage}{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{algo_comparison_sssp}
    (b) sssp
    \end{minipage}
    \begin{minipage}{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{algo_comparison_cc}
    (c) cc
    \end{minipage}
   % \end{minipage}
    \caption{Execution time of different variants of algorithm in Galois \xpointshortend.}
    \label{fig:res:algo_variant_plot}
\end{figure}

In shared memory graph analytics, memory accesses are an
important factor in determining the performance of the algorithm. The two
important considerations for performant algorithms are
(a) reducing the cost of memory accesses and (b) reducing the number of memory
accesses by employing work efficient algorithms. We have discussed various
factors contributing to and the benefits of reducing the memory access cost
in Section~\ref{subsec:3dxpoint_setup}. In this section, we will analyze the
importance of using work efficient algorithms to reduce the number of memory
accesses.

\todo{I (Loc) drafted this, please make a pass/revision}

Figure~\ref{fig:res:algo_variant_plot} shows the execution time of different
variants of bfs, cc, and sssp on \xpointshortend with three graphs. clueweb12
and wdc12 are high-diameter graphs while rmat32 is a low-diameter graph.

In all algorithms and graphs, the dense worklist variant of
the algorithm is never the best performing version. This is because the
dense worklist is an implicit worklist that requires iterating over all vertices
of a graph to determine if there is work to be done. This increases the
amount of memory accesses, thus hurting performance.

% TODO this paragraph needs refining
\todo{This paragraph is wordy, please revise. -Loc}
For bfs, direction optimization~\cite{dobfs} performs well for rmat32,
a low-diameter graph, but for high-diameter graphs, surprisingly enough,
it is outperformed by a
sparse worklist implementation where active vertices are stored in an
explicit worklist (this reduces memory accesses compared to the dense worklist
variant since it does not traverse the entire graph). The reason for this
is that direction optimization must make many more
accesses since it has both incoming and outgoing edges unlike the
sparse worklist implementation which only uses outgoing edges.
High-diameter graphs have a long tail and a large amount of iterations
the benefits of direction optimization are not enough to outweigh the
additional memory access overhead it incurs when the amount of iterations
over the graph is large.

For sssp, the delta-stepping algorithm significantly outperforms the dense
worklist. This is because delta-stepping reduces the overall amount
of work to be done since it reduces redundant work by limiting active
nodes: less work means less memory accesses, which increases performance.

For cc, label propagation combined with shortcutting~\cite{shortcutcc} performs
best because a node can quickly propagate a connected component label by
sending it to nodes that are not necessarily its neighbors, thereby reducing
the total amount of work that occurs. Pointer jumping cc also reduces
the amount of work, but the benefits only show themselves for very
high-diameter graphs like wdc12.

Note that these findings do not apply only to \xpointshortend: \todo{Figure
DRAM figure here} shows the same experiments conducted on a large DRAM machine
with enough memory to fit these graphs. The same general principles apply:
algorithms that make a low amount of memory accesses perform better than ones
that make a higher amount of accesses.
\todo{verify this is correct}
Additionally, it is important to note that work-efficient algorithms such as
cc's label propagation with shortcutting cannot be expressed as a vertex
program. Therefore, for good performance on large-memory machines,
graph analytics frameworks must be flexible enough to express many kinds
of algorithms that are not just vertex programs.

To conclude, we show that work-efficient algorithms that can reduce the
total amount of memory accesses are important for running on graph
algorithms \xpointshort (and large memory systems) with good performance,
particularly for graphs with high-diameter.


==> tbl_inputs_transpose.tex <==
\begin{table}[t]
\footnotesize
\centering

\begin{tabular}{@{}l@{\hskip1.8pt}r@{ }r@{ }r@{ }r@{ }r@{}r@{ }r@{ }r@{ }r@{}}
\toprule
                               & \textbf{kron30}    & \textbf{clueweb12}       & \textbf{uk14}    & \textbf{rmat32}    & \textbf{wdc12}                   \\
\midrule                                                                                                                                             
\textsf{$|V|$}                 & 1,073M             & 978M                      & 788M            & 4295M               & 3,563M                           \\
\textsf{$|E|$}                 & 10,791M            & 42,574M                   & 47,615M         & 68,719M              & 128,736M                         \\
\textsf{$|E|/|V|$}             & 16                 & 44                        & 60.4            & 16                  & 36                               \\
\textsf{max $D_{out}$}         & 3.2M               & 7,447                     & 16,365          & 10.4M             & 55,931                           \\
\textsf{max $D_{in}$}          & 3.2M               & 75M                            & 8.6M       & 10.4M                     & 95M                              \\
\textsf{Est. diameter}         & 6                   & 498                       & 2498           & 7                   &  5274                                 \\
\textsf{Size (GB)}             & 136                 &325                        & 361             &  544                &986                              \\
\bottomrule
\end{tabular}
\caption{Inputs and their key properties.}
%\vspace{-5pt}
\label{tbl:inputs}
\vspace{-5pt}
\end{table}


\begin{table}[t]
    \footnotesize
    \centering
    
    \begin{tabular}{@{}l@{\hskip1.8pt}r@{ }r@{ }r@{ }r@{ }r@{}r@{ }r@{ }r@{ }r@{}}
    \toprule
                                   & \textsf{$|V|$}    & \textsf{$|E|$}       & \textsf{$|E|/|V|$}    & \textsf{max $D_{out}$}     & \textsf{max $D_{in}$} & \textsf{Est. diameter} &  \textsf{Size (GB)}                  \\
    \midrule                                                                                                                                             
    \textbf{kron30}                 & 1,073M             & 978M                      & 788M            & 4295M               & 3,563M                           \\
    \textbf{clueweb12}                 & 10,791M            & 42,574M                   & 47,615M         & 68,719M              & 128,736M                         \\
    \textbf{uk14}             & 16                 & 44                        & 60.4            & 16                  & 36                               \\
    \textbf{iso_m100}         & 3.2M               & 7,447                     & 16,365          & 10.4M             & 55,931                           \\
    \textbf{max $D_{in}$}          & 3.2M               & 75M                            & 8.6M       & 10.4M                     & 95M                              \\
    \textsf{Est. diameter}         & 6                   & 498                       & 2498           & 7                   &  5274                                 \\
    \textsf{Size (GB)}             & 136                 &325                        & 361             &  544                &986                              \\
    \bottomrule
    \end{tabular}
    \caption{Inputs and their key properties.}
    %\vspace{-5pt}
    \label{tbl:inputs}
    \vspace{-5pt}
    \end{table}

==> tbl_numa_migration.tex <==
%\begin{table}[t]
\footnotesize
\centering
%\caption{Data TLB misses (Load + Store) and page migrations for bfs with small (4KB) page size for large real-world input graphs on \xpointshortend.}
(a) {Small pages (4KB)}
%\label{tbl:numa_migration}

%\begin{tabular}{lllll}
\begin{tabular}{@{ }l|@{\hskip1.8pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r}
%\begin{tabular}{@{  }l@{\hskip4pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}}
\toprule
          & \multicolumn{3}{c|}{NUMA Migrations On}& \multicolumn{3}{|c}{NUMA Migrations Off}  \\
\cline{2-7}
          & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}DTLB\\misses\end{tabular}}     & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}Pages\\migrated\end{tabular}} & \multicolumn{1}{r|}{ \begin{tabular}[c]{@{}l@{}}\% local\\access\end{tabular}}  & \multicolumn{1}{|r}{ \begin{tabular}[c]{@{}l@{}}DTLB\\ misses\end{tabular}}     & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}Pages\\migrated\end{tabular}}  & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}\% local\\access\end{tabular}}          \\
\midrule
clueweb12 & 303.5M       &7.9M   &\multicolumn{1}{r|}{51.3\%}                 & \multicolumn{1}{|r}{138.7M}      &0       &50.9\%                 \\
uk14& 116.9M       &11.0M   &\multicolumn{1}{r|}{52.9\%}                 & \multicolumn{1}{|r}{65.9M}      &0       &52.2\%                 \\
wdc12     & 251.0M         &28.2M  &\multicolumn{1}{r|}{49.3\%}                & \multicolumn{1}{|r}{144.5M}      &0       &50.5\%                 \\
\bottomrule
\end{tabular}
%\vspace{-10pt}
%\end{table}


==> tbl_numa_migration_combined.tex <==
%\begin{table}[t]
\footnotesize
\centering
%\caption{Data TLB misses (Load + Store) and page migrations for bfs with small (4KB) page size for large real-world input graphs on \xpointshortend.}
%\label{tbl:numa_migration}

%\begin{tabular}{lllll}
\begin{tabular}{@{ }l|@{\hskip1.8pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r}
%\begin{tabular}{@{  }l@{\hskip4pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}}
\toprule
          & \multicolumn{6}{c|}{Small pages (4KB) } & \multicolumn{6}{|c}{Huge pages (2MB) } \\
\cline{2-13}
          & \multicolumn{3}{c|}{NUMA Migrations On}& \multicolumn{3}{|c|}{NUMA Migrations Off}& \multicolumn{3}{|c|}{NUMA Migrations On}& \multicolumn{3}{|c}{NUMA Migrations Off}  \\

\cline{2-13}
          & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}DTLB\\misses\end{tabular}}     & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}Pages\\migrated\end{tabular}} & \multicolumn{1}{r|}{ \begin{tabular}[c]{@{}l@{}}\% local\\access\end{tabular}}  & \multicolumn{1}{|r}{ \begin{tabular}[c]{@{}l@{}}DTLB\\ misses\end{tabular}}     & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}Pages\\migrated\end{tabular}}  & \multicolumn{1}{r|}{ \begin{tabular}[c]{@{}l@{}}\% local\\access\end{tabular}}    & \multicolumn{1}{|r}{ \begin{tabular}[c]{@{}l@{}}DTLB\\misses\end{tabular}}     & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}Pages\\migrated\end{tabular}} & \multicolumn{1}{r|}{ \begin{tabular}[c]{@{}l@{}}\% local\\access\end{tabular}}  & \multicolumn{1}{|r}{ \begin{tabular}[c]{@{}l@{}}DTLB\\ misses\end{tabular}}     & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}Pages\\migrated\end{tabular}}  & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}\% local\\access\end{tabular}}      \\
\midrule
  clueweb12           & 303.5M      &7.9M         &\multicolumn{1}{r|}{51.3\%}                 & \multicolumn{1}{|r}{138.7M}      &0       & \multicolumn{1}{l|}{50.9\%}        & \multicolumn{1}{|r}{38.9M}       &575   &\multicolumn{1}{r|}{50.5\%}                 & \multicolumn{1}{|r}{43.1M}      &0       &49.0\%             \\
  uk14                & 116.9M      &11.0M        &\multicolumn{1}{r|}{52.9\%}                 & \multicolumn{1}{|r}{65.9M}      &0       &\multicolumn{1}{l|}{52.2\%}         &  \multicolumn{1}{|r}{6.0M}       &504   &\multicolumn{1}{r|}{53.3\%}                 & \multicolumn{1}{|r}{5.9M}      &0       &49.5\%              \\
  wdc12               & 251.0M      &28.2M        &\multicolumn{1}{r|}{49.3\%}                & \multicolumn{1}{|r}{144.5M}      &0       &\multicolumn{1}{l|}{50.5\%}        &  \multicolumn{1}{|r}{67.0M}       &723  &\multicolumn{1}{r|}{53.5\%}                & \multicolumn{1}{|r}{76.9M}      &0       &53.0\%              \\
\bottomrule
\end{tabular}
%\vspace{-10pt}
%\end{table}


==> tbl_numa_migration_huge_pages.tex <==
%\begin{table}[t]
\footnotesize
\centering
%\caption{Data TLB misses (Load + Store) and page migrations for bfs with huge (2MB) page size for large real-world input graphs on \xpointshortend.}
(b) {Huge pages (2MB)}
%\label{tbl:numa_migration}

%\begin{tabular}{lllll}
\begin{tabular}{@{}l|@{\hskip1.8pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r@{\hskip0pt}r}
%\begin{tabular}{@{  }l@{\hskip4pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}}
\toprule
          & \multicolumn{3}{c|}{NUMA Migrations On}& \multicolumn{3}{|c}{NUMA Migrations Off}  \\
\cline{2-7}
          & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}DTLB\\misses\end{tabular}}     & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}Pages\\migrated\end{tabular}} & \multicolumn{1}{r|}{ \begin{tabular}[c]{@{}l@{}}\% local\\access\end{tabular}}  & \multicolumn{1}{|r}{ \begin{tabular}[c]{@{}l@{}}DTLB\\ misses\end{tabular}}     & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}Pages\\migrated\end{tabular}}  & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}\% local\\access\end{tabular}}          \\
\midrule
clueweb12       & 38.9M       &575   &\multicolumn{1}{r|}{50.5\%}                 & \multicolumn{1}{|r}{43.1M}      &0       &49.0\%                 \\
uk14            & 6.0M       &504   &\multicolumn{1}{r|}{53.3\%}                 & \multicolumn{1}{|r}{5.9M}      &0       &49.5\%                 \\
wdc12           & 67.0M       &723  &\multicolumn{1}{r|}{53.5\%}                & \multicolumn{1}{|r}{76.9M}      &0       &53.0\%                 \\
\bottomrule
\end{tabular}
%\vspace{-10pt}
%\end{table}


==> tbl_page_size_tlb_misses.tex <==
\begin{table}[t]
\footnotesize
\centering
  \caption{Number of pages, Data TLB misses (Load + Store) and CPU cycles spent in Page Walking (PW) for small (4KB) and huge (2MB) page sizes for bfs for large real-world input graphs on \xpointshort with NUMA migrations off.}
\label{tbl:page_size_counters}

%\begin{tabular}{lllll}
\begin{tabular}{@{ }l|@{\hskip1.8pt}r@{\hskip3pt}r@{\hskip3pt}r@{\hskip3pt}r@{\hskip3pt}r@{\hskip3pt}r@{\hskip3pt}r@{\hskip3pt}}
%\begin{tabular}{@{  }l@{\hskip4pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}}
\toprule
& \multicolumn{3}{c|}{Small pages (4KB)}& \multicolumn{3}{|c}{Huge pages (2MB)}  \\
\cline{2-7}
          &  \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}Total\\ pages\end{tabular}}   &  \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}DTLB\\ misses\end{tabular}}   & \multicolumn{1}{r|}{ \begin{tabular}[c]{@{}l@{}}Cycles\\ for PW\end{tabular}}     &  \multicolumn{1}{|r}{ \begin{tabular}[c]{@{}l@{}}Total\\ pages\end{tabular}}   &  \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}DTLB\\ misses\end{tabular}}   & \multicolumn{1}{r}{ \begin{tabular}[c]{@{}l@{}}Cycles\\ for PW\end{tabular}}         \\
\midrule
clueweb12 &   43.6M       & 138.7M        &\multicolumn{1}{r|}{23.4B}                        & \multicolumn{1}{|r}{0.085M}          & 43.1M               & 3.2B                 \\
uk14      &   48.1M          & 65.9M        &\multicolumn{1}{r|}{16.2B}                        & \multicolumn{1}{|r}{0.094M}          & 5.9M               & 1.3B                 \\
wdc12     &   132.8M     & 144.5M        &\multicolumn{1}{r|}{47.7B}                        & \multicolumn{1}{|r}{0.26M}          & 76.9M               & 5.4B                 \\
\bottomrule
\end{tabular}
%\vspace{-10pt}
\end{table}


==> vldb_rebuttal.tex <==
We thank the reviewers for their feedback. We have incorporated their suggestions in
the revised submission. 
In this response, we first list the revisions we made to 
the paper and then our response 
to each question or comment from the reviewers. 
The revised paper follows our response.\\

\noindent{\textbf{\large Revisions Made to the Paper}}\\

\revise{Major changes to the paper or parts that we want to emphasize have been
highlighted in blue in the paper}. 
The main changes made to address reviewer comments are below. 
% In the rest of this response, 
% they will be referred to via R1, R2, R3, etc. for the
% corresponding numbered point below.

\begin{enumerate}

\item The justification for our selection of 
shared-memory, distributed-memory, and out-of-core 
graph frameworks has been made more
clear in Sections~\ref{subsec:framework_comparison}, 
\ref{subsec:xpoint_vs_stampeded}, 
and~\ref{subsec:outofcore} respectively.

\item We evaluated a large protein dataset 
(see (iso\_m100~\cite{protein}) in Table~\ref{tbl:inputs}). 
Figure~\ref{fig:res:other_vs_galois}(c) and 
Table~\ref{tbl:stampvsoptane} present results 
for this graph.

% \item Added text and rewrote some text throughout the paper to make it easier
% to understand technical terms and concepts that were unclear before throughout
% the paper

\item Technical terms and concepts used in the paper are supplemented with more descriptions
for ease of understanding.

\item We added citations to graph algorithms throughout the paper; 
due to lack of space, we are not able to describe these algorithms.

\item We added more clear motivation(s) 
and takeaway(s) for each subsection in Section~\ref{sec:results}.

\item We briefly discussed cost and ease of use of Optane in Section~\ref{subsec:summary}.
% Optane lets users run shared-memory frameworks out-of-the-box and 
% is a cheaper technology than both DRAM and distributed clusters.

\item Future challenges in the area are briefly mentioned in
Section~\ref{subsec:summary}.
% techniques should be developed to increase
% near-memory hit rate and more studies into app-direct mode need to
% be conducted

\item We added discussion on strong scaling of 
graph analytics applications on 
Optane PMM in Section~\ref{subsec:xpoint_vs_dram} 
and on weak scaling in Section~\ref{subsec:xpoint_vs_stampeded}.

\item We added discussion on generalization of Optane use to other kinds of graph
applications (e.g., graphs with attributes) in Section~\ref{subsec:summary}.

\end{enumerate}

% We address specific points next.\\

\noindent{\textbf{\large General}}\\

\noindent{\textbf{Q1:
What are the advantages of Optane, and why use it for graph analytics?}}

Optane is a recently developed memory technology from Intel that is a cheaper
alternative to DRAM.  Its latency is higher than that of DRAM but much lower
than that of SSD.  It allows a single machine to have up to 6TB of main memory,
allowing it to run memory-hungry applications (in memory mode) without
substantial reworking of algorithms and implementations needed by
distributed-memory or out-of-core processing.  Graph analytics on ever-growing
massive graphs is one such application.  In this paper, we empirically study
the viability of Optane to process massive graphs on a single machine.

% Optane provides a cheaper alternative to DRAM; although it is slower in latency
% to DRAM, it provides faster speed than a solid-state drive (SSD). In addition,
% it can act as both as main memory via its memory mode or as secondary storage
% via app direct mode (see Section~\ref{3dxpoint}. This, in particular, is
% extremely powerful as it allows any application to run transparently using
% Optane as main memory or secondary storage \emph{without any changes required
% to the application}.

% Optane does not provide anything specific to graph analytics.  However, as
% graphs are becoming extremely large, analyzing large graphs would require an
% out-of-core or distributed graph analytics system which both have their
% associated overheads. Optane allows users to run shared-memory graph systems
% without any changes, and, more importantly, without any of the overheads
% associated with out-of-core or distributed execution.  

As Optane is a new technology, our paper provides a study of \emph{how} graph
analytics systems should be run for best performance on Optane.  It also
analyzes different algorithms for multiple graph analytics problems on massive
real-world datasets and gives recommendations for choosing an algorithm, that
not only apply to Optane but also to large DRAM systems.  We also
quantitatively show that performance of graph analytics on Optane can be
competitive or better than that on distributed or out-of-core systems. 
\\

% as the best system to use for graph
% analytics since there are cases where distributed clusters have advantages
% (e.g., more compute power): instead, we argue that Optane is a \emph{viable
% alternative} for fast graph analytics.

\noindent{\textbf{Q2: 
Why did you evaluate the graph frameworks that you did and not others?}}

The justification for our selection of 
shared-memory, distributed-memory, and out-of-core 
graph frameworks has been made more
clear in Sections~\ref{subsec:framework_comparison}, 
\ref{subsec:xpoint_vs_stampeded}, 
and~\ref{subsec:outofcore} respectively.

On shared-memory architectures, we chose GAP, GraphIt, Galois, and GBBS because
they exemplify different approaches in terms of the trade-off between
programming effort and performance.  They are widely used and cited by other
works in graph analytics.  Moreover, their source code is robust and
well-maintained.

On the distributed cluster, we evaluated D-Galois because it is the
state-of-the-art distributed graph analytics system.  Dathathri et
al.~\cite{gluon} show that D-Galois is much faster than Gemini~\cite{gemini}
(especially at scale) and Zhu et al.~\cite{gemini} show that Gemini is much
faster than older systems like GraphX~\cite{graphx},
PowerGraph~\cite{powergraph}, and PowerLyra~\cite{powerlyra} (PowerLyra extends
GraphLab~\cite{graphlab} to make it faster).  Dathathri et al.~\cite{phoenix}
also show that D-Galois (called Phoenix in~\cite{phoenix}) is an order of
magnitude or more faster than GraphX while providing the same level of fault
tolerance.

For out-of-core frameworks, we chose GridGraph because it is the
state-of-the-art out-of-core graph analytics system.  Some recent out-of-core
graph analtyics works like Wonderland~\cite{wonderland} and Lumos~\cite{lumos}
are faster than GridGraph but they only handle a subset of algorithms that
GridGraph handles (Lumos is for topology-driven algorithms only and Wonderland
is for path-based algorithms, like bfs, only).  They are at the most an order
of magnitude faster than GridGraph.  As Table~\ref{tbl:outofcore} shows, Galois
is more than two orders of magnitude faster than GridGraph, so we expect these
specialized frameworks to not be as fast as Galois on Optane.
\\

\noindent{\textbf{\large Reviewer 1}}\\

% vision paper, not experimental paper
\noindent{\textbf{D1: More suited for vision, not experimental track?}}

We believe our paper is an extensive experimental study and 
is a good fit for the experimental track. 
It is not a vision paper because we are not introducing a 
new hardware technology 
(anyone can buy the Optane system from Intel). 
As mentioned in response to Q1, 
Optane is a recently developed memory technology and 
we empirically study the viability of Optane to 
analyze massive graphs.

In Section~\ref{sec:results}, 
we compare many (shared-memory, out-of-core, and
distributed-memory) graph analytics frameworks 
across many different platforms, in order to evaluate the
advantages and disadvantages of: 
(1) various shared-memory graph analytics frameworks for
Optane and large memory systems (Section~\ref{subsec:framework_comparison}),
(2) shared-memory and distributed-memory graph analytics with regard
to the differences in expressibility and the performance implications of the
differences (Section~\ref{subsec:xpoint_vs_stampeded}), and (3) shared-memory
and out-of-core graph analytics
(Section~\ref{subsec:outofcore}). This is all done in the context of Optane,
which makes this analysis possible by providing 6TB of memory that can be
transparantly used as either main memory or secondary storage by shared-memory and 
out-of-core frameworks, respectively. 

In addition, Section~\ref{sec:abstractions}
compares different algorithmic choices 
for many graph analytics problems 
on large memory systems using massive real-world datasets. 
Section~\ref{sec:mem-access} evaluates 
different system knobs on Optane that need to be tuned 
to get good performance for graph analytics.

Although done in the context of Optane, \emph{the conclusions of Sections~\ref{subsec:algo_design} and~\ref{sec:results}
do not only apply to Optane but rather to large memory systems in general}. 
Our experimental evaluation has key lessons 
for designers of algorithms, frameworks, and architectures 
of graph analytics.
\\

% Concepts/technical terms not explained
\noindent{\textbf{D2: Concepts/technical terms not explained.}}
% Formally define graph problems
\\
\noindent{\textbf{D4: Architectural details need explanation.}}

Technical terms and concepts used in the paper are supplemented with more descriptions
for ease of understanding.
\\

\noindent{\textbf{D3: Formal definition of graph problems needed.}}
% Architectural detail/clarification

We added citations to graph algorithms throughout the paper; 
due to lack of space,
we are not able to describe these algorithms.
\\

% Use other real world networks
\noindent{\textbf{D5: Graphs from other domains of graphs.}}

We evaluated a large protein dataset 
(see (iso\_m100~\cite{protein}) in Table~\ref{tbl:inputs}). 
Figure~\ref{fig:res:other_vs_galois}(c) and 
Table~\ref{tbl:stampvsoptane} present results 
for this graph.

% Note that 
% most real-world datasets are not large enough to
% warrant running on large DRAM machines or on Optane. 
We are using the largest
publicly available graphs that currently exist. 
Many datasets from other domains are not public.  
If they are, they fit (using CSR format) in the 384 GB DRAM 
of the Optane system that we use in our study.
In other words, we could not find graphs in other domains 
(like road networks) that are public and 
that do not fit in the DRAM 
of the Optane system. 
\\

%Experimental comparison does not seem fair as different platforms/compilers
%used for different settings
\noindent{\textbf{D6: Experimental comparison among different platforms
does not seem fair.}}

Optane vs. Entropy (large DRAM machine): The point of the comparison was not a
head-to-head comparison to show that one hardware or system 
is better than the other. Instead,
this comparison was mainly to show that our observations and suggestions
for running graph analytics efficiently on Optane \emph{also apply to large
memory systems}.
%  (2) the overhead of running on Optane is not high if
% near-memory cache is used effectively.

Optane vs. Distributed Cluster: The purpose of the comparison between Optane
and the distributed cluster 
was to test whether Optane is a viable alternative 
(not a replacement) to 
distributed clusters for fast analysis of massive graphs. 
In other words, 
our intention was to test whether 
graph analytics on Optane can be
competitive with graph analytics on a cluster in terms of performance. 
For logistical reasons (Stampede2 is a public distributed cluster), 
it is difficult to ensure
that both platforms use the exact same resources (threads and memory). 
We attempt a fair comparison by limiting the resources used
on both platforms.
% We conducted experiments where we use the same amount of compute resources
% (threads) on both machines, and 
We also show that even when the
distributed cluster uses significantly more resources (i.e.,
256 machines), Optane is still competitive in many cases. 
% Note that we do not think the compiler version difference 
% between the platforms will impact our observations. 
\\

% Motivations/takeaways for each experimental sectoin
\noindent{\textbf{D7: Motivations/takeaways should be clear
for each experimental section.}}

We added more clear motivation(s) 
and takeaway(s) for each subsection in Section~\ref{sec:results}.
\\

% Discussion on cost, user friendliness, etc.
\noindent{\textbf{D8: Discussion on cost/user friendliness.}}

We briefly discussed cost and ease of use of Optane in Section~\ref{subsec:summary}.
% Optane lets users run shared-memory frameworks out-of-the-box and 
% is a cheaper technology than both DRAM and distributed clusters.
\\

% Benefits of Optane, also why it is suitable for graphs
\noindent{\textbf{D9: Optane benefits + why suitable
for graphs?}}

See the response to Q1 above.
\\

% Dist cluster systems, why no GraphX, Giraph, GraphLab
\noindent{\textbf{D10: What about other distributed graph analytics systems like
GraphX, Giraph, GraphLab?}} 

See the response to Q2 above.
\\

% Challneges/future directions
\noindent{\textbf{D11: Challenges/future directions?}}

Future challenges in the area are briefly mentioned in
Section~\ref{subsec:summary}.
% techniques should be developed to increase
% near-memory hit rate and more studies into app-direct mode need to
% be conducted
\\

\noindent{\textbf{\large Reviewer 3}}\\

% Focus is mostly on memory tuning and hardware variations
\noindent{\textbf{W1: Focus is mostly on memory tuning and hardware
variations.}}

Section~\ref{sec:abstractions} details the importance of algorithm design and
the expressibility of graph analytics systems. In particular, it shows the
important of asynchronous, data-driven algorithms that can use non-vertex
operators by showing that these algorithms are more efficient than other
algorithms. Section~\ref{subsec:framework_comparison} also shows that Galois
has advantages over other systems in part to being able to use non-vertex
operators and execute asynchronously.
\\

% justification of graph framework selection
\noindent{\textbf{W2: Justify the graph framework selection.}}

See the response to Q2 above.
\\

%* Some results show Optane does not have advantage over compared setup.
%Considering effort for tuning NUMA, the advantage of Optane remain limited for
%certain cases. 
\noindent{\textbf{W3: Optane is not always best.}}
\\
\noindent{\textbf{Why Optane with graphs analytics?}}

See the response to Q1 above.\\
\\

\noindent{\textbf{\large Reviewer 4}}\\

\noindent{\textbf{Q1: Scale-out performance of Optane PMM?}}

% \todo{refer to changes in the paper}
We added discussion on strong scaling of 
graph analytics applications on 
Optane PMM in Section~\ref{subsec:xpoint_vs_dram}
and on weak scaling in Section~\ref{subsec:xpoint_vs_stampeded}.

Figure~\ref{fig:res:dram_vs_xpoint} 
shows the strong scaling of many graph analytics applications 
on input graphs that fit in both DRAM and Optane. 
It is clear that all applications 
scale well on all inputs (except kcore on clueweb12) 
as the number of threads are increased. 
More importantly, the strong scaling is similar whether 
DRAM or Optane is used as main memory. 

Table~\ref{tbl:stampvsoptane} shows the performance 
of many graph analytics applications on Optane 
for input graphs of different sizes (smallest to largest). 
Most applications take more time for larger graphs. 
Although wdc12 is $\sim3\times$ larger (in terms of edges) 
than clueweb12, 
kcore and pr take less time on wdc12 than clueweb12, 
but the other applications take on average $\sim7\times$ 
more time on wdc12 than clueweb12. 
This provides an estimate for the weak scaling of these 
applications.

We also measured the performance of all applications on 8 
and 96 threads of the Optane system (using Optane memory). 
The geo-mean speedup of all applications 
on 96 threads over 8 threads 
is $4.3\times$, $4.2\times$, $4.7\times$, and $3.5\times$ 
for kron30, clueweb12, uk14, and wdc12 respectively. 
Thus, the strong scaling speedup does not vary by much 
as the size of the graph grows.
% Our results show that Optane still performs well as the graphs used on
% it get larger. Care must be taken, however, to account for near-memory
% as shown Sections~\ref{sec:mem-access} and~\ref{subsec:xpoint_vs_dram}:
% near-memory cache misses must be reduced for good performance, and
% that becomes difficult to do as graphs grow in size.
\\

\noindent{\textbf{Q2: Discussuion on graphs with attributes.}}

We added discussion on generalization of Optane use to other kinds of graph
applications (e.g., graphs with attributes) in Section~\ref{subsec:summary}.
\\

